GENIEx: A Generalized Approach to Emulating Non-Ideality in Memristive Xbars using Neural Networks

The analog nature of computing in Memristive crossbars poses significant issues due to various non-idealities such as: parasitic resistances, non-linear I-V characteristics of the device etc. The non-idealities can have a detrimental impact on the functionality i.e. computational accuracy of crossbars. Past works have explored modeling the non-idealities using analytical techniques. However, several non-idealities have data dependent behavior. This can not be captured using analytical (non data-dependent) models thereby, limiting their suitability in predicting application accuracy. To address this, we propose a Generalized Approach to Emulating Non-Ideality in Memristive Crossbars using Neural Networks (GENIEx), which accurately captures the data-dependent nature of non-idealities. We perform extensive HSPICE simulations of crossbars with different voltage and conductance combinations. Following that, we train a neural network to learn the transfer characteristics of the non-ideal crossbar. Next, we build a functional simulator which includes key architectural facets such as \textit{tiling}, and \textit{bit-slicing} to analyze the impact of non-idealities on the classification accuracy of large-scale neural networks. We show that GENIEx achieves \textit{low} root mean square errors (RMSE) of $0.25$ and $0.7$ for low and high voltages, respectively, compared to HSPICE. Additionally, the GENIEx errors are $7\times$ and $12.8\times$ better than an analytical model which can only capture the linear non-idealities. Further, using the functional simulator and GENIEx, we demonstrate that an analytical model can overestimate the degradation in classification accuracy by $\ge 10\%$ on CIFAR-100 and $3.7\%$ on ImageNet datasets compared to GENIEx.

==> design-param.tex <==

% \begin{tabularx}{\columnwidth}{|X|X|X|X|}
%     \hline
%     \multicolumn{2}{|c|}{Design Parameter}          & \multicolumn{2}{c|}{Value}                                   \\ \hline\hline
%     \multicolumn{2}{|c|}{Crossbar Size}             & \multicolumn{2}{c|}{16, 32, 64}                              \\ \hline
%     \multicolumn{2}{|c|}{ON Resistance}             & \multicolumn{2}{c|}{50k$\Omega$, 100k$\Omega$, 300k$\Omega$} \\ \hline
%     \multicolumn{2}{|c|}{ON/OFF Ratio}              & \multicolumn{2}{c|}{2, 6, 10}                                \\ \hline \hline
%     Non-ideality Parameters & Value                 & Device Parameters \cite{
%     xu2014modeling, yu2012neuromorphic}             & Value               \\ \hline
%     $R_{source}$            & 500/1000 $\Omega$     & $d_0$                                  & 0.25 nm             \\ \hline
%     $R_{sink}$              & 100/500 $\Omega$      & $V_0$                                  & 0.25 V              \\ \hline
%     $R_{wire}$              & 2.5 $\Omega$ per cell & $I_0$                                  & 0.1 mA              \\ \hline
% \end{tabularx}
